ToSA: Token Selective Attention for Efficient Vision Transformers

In this paper, we propose a novel token selective attention approach, ToSA, which can identify tokens that need to be attended as well as those that can skip a transformer layer. More specifically, a token selector parses the current attention maps and predicts the attention maps for the next layer, which are then used to select the important tokens that should participate in the attention operation. The remaining tokens simply bypass the next layer and are concatenated with the attended ones to re-form a complete set of tokens. In this way, we reduce the quadratic computation and memory costs as fewer tokens participate in self-attention while maintaining the features for all the image patches throughout the network, which allows it to be used for dense prediction tasks. Our experiments show that by applying ToSA, we can significantly reduce computation costs while maintaining accuracy on the ImageNet classification benchmark. Furthermore, we evaluate on the dense prediction task of monocular depth estimation on NYU Depth V2, and show that we can achieve similar depth prediction accuracy using a considerably lighter backbone with ToSA.

==> sec/2_related.tex <==
\section{Related Works}
\label{sec:related}
\vspace{-3pt}

Even since its introduction~\cite{dosovitskiy2020image}, vision transformers have been extensively studied and utilized for various computer vision tasks, including classification, detection, segmentation, depth estimation, tracking, 3D reconstruction, and more. We refer readers to these surveys for a more comprehensive coverage of these works. 

Since the self-attention operation incurs quadratic computation and memory costs w.r.t. the number of input tokens, several papers have looked into how to reduce the number of tokens going into the attention computation~\cite{}. Most of these works, however, focus on the image classification and discard tokens that are deemed less important as features are computed by the neural network layers. While this works for classification as it only requires a final classification decision, models developed with such approaches cannot be used as backbones for dense prediction tasks, which requires a prediction value on every pixel location. 
Token merging for fast stable diffusion, however, this requires extra token un-merging steps, which creates additional costs.

==> sec/6_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
